Partial Identifiability in Discrete Data With Measurement Error

When data contains measurement errors, it is necessary to make assumptions relating the observed, erroneous data to the unobserved true phenomena of interest. These assumptions should be justifiable on substantive grounds, but are often motivated by mathematical convenience, for the sake of exactly identifying the target of inference. We adopt the view that it is preferable to present bounds under justifiable assumptions than to pursue exact identification under dubious ones. To that end, we demonstrate how a broad class of modeling assumptions involving discrete variables, including common measurement error and conditional independence assumptions, can be expressed as linear constraints on the parameters of the model. We then use linear programming techniques to produce sharp bounds for factual and counterfactual distributions under measurement error in such models. We additionally propose a procedure for obtaining outer bounds on non-linear models. Our method yields sharp bounds in a number of important settings -- such as the instrumental variable scenario with measurement error -- for which no bounds were previously known.

==> markov_chain.tex <==
% \documentclass[main.tex]{subfiles}
%
% \begin{document}

	
\subsection{Multiple proxies with unconfounded measurement error}
\label{sec:markov-chain}

In certain setting, we may be willing to assume the $A$ is fully independent of
$Y$ given $X$ as shown in Figure \ref{fig:iv} (b). In this case, the inequality
constraints implied by the exclusion restriction are replaced by equality
constraints implied by the Markov chain assumption, specifically: $\phi_{xya}
\sum_{a',y'} \phi_{xy'a'} = (\sum_{y'} \phi_{xy'a}) (\sum_{a'} \phi_{xya'})$.
Unfortunately, this conditional independence assumption is a quadratic function
of $\phi$ and we are no longer presented with a LP. While valid non-sharp
bounds may be derived for this case by relaxing the modeling assumptions to
those in Figure \ref{fig:iv} (a), the sharp bounds may be substantially tighter.

Obtaining such bounds for the general case is difficult as, in general,
quadratic programming is NP-hard \cite{pardalos1991quadratic}; however, certain
special cases may still amenable to analysis. In particular, for binary
$X$ and $Y$, we have:

\begin{proposition}
    \label{prop:binary_bounds}
	%
    Let $X$ and $Y$ be binary variables such that $X \not\independent Y$, let
    $A$ be a discrete variable such that $A \independent Y | X$ and $P(A=a) >
    0$ for all $a$, and let $p_y = P(Y=y)$ and $p_{y \mid a} = P(Y=y\mid A=a)$.
    Then we have the following sharp bounds on $P(X=1)$:
	%
    \begin{align}
	  %       P(X=1) &\in [l,u] \cup [1-u,1-l]\\ \nonumber
	  % l &= \max_a \frac{P(Y=1) - P(Y=1|A=a)}{1 - P(Y=1|A=a)}\\ \nonumber
	  % u &= \min_a \frac{P(Y=1)}{P(Y=1|A=a)}
	  P(X=1) &\in \bigcup_{y\in\{0,1\}} \left[\frac{p_y - \min_a p_{y \mid a}}{1 - \min_a p_{y \mid a}},\frac{p_y}{\max_a p_{y\mid a}}\right]
    \end{align}
\end{proposition}
%
See Appendix \ref{app:prop_1_proof} for a complete proof. So long as the mutual
information between $A$ and $Y$ is non-zero, Proposition \ref{prop:binary_bounds}
bounds $P(X=1)$ away from zero and one; however, when the mutual information
between $A$ and $Y$ is sufficiently high, $P(X=1)$ is also bounded away from
$\frac{1}{2}$. For example, in the extreme case where $A$ uniquely determines
$Y$, we have $P(X=1) \in \left\{p_0,p_1\right\}$. More generally, we can bound
$P(X=1)$ away from $\frac{1}{2}$ any time $2 p_1 < \max_a p_{1|a}$ or $2 p_1 >
1-\min_a p_{1|a}$. As above, these bounds can be combined with other common
measurement error assumptions and some examples are presented in Appendix
\ref{app:combinations_with_markov}.
% These bounds can also be generalized to continuous $A$ by substituting sup/inf
% for max/min and densities for masses where appropriate; however, estimating
% $p(Y|A)$ becomes much harder for continuous (or high-dimensional) $A$.
In the following section, we extend our earlier discussion of potential
outcomes to consider partial identification bounds for causal parameters and
constraints relating multiple potential outcomes.

% \end{document}

